Asynchronous Anytime Sequential Monte Carlo

We introduce a new sequential Monte Carlo algorithm we call the particle cascade. The particle cascade is an asynchronous, anytime alternative to traditional particle filtering algorithms. It uses no barrier synchronizations which leads to improved particle throughput and memory efficiency. It is an anytime algorithm in the sense that it can be run forever to emit an unbounded number of particles while keeping within a fixed memory budget. We prove that the particle cascade is an unbiased marginal likelihood estimator which means that it can be straightforwardly plugged into existing pseudomarginal methods.

==> approach.tex <==
% !TEX root =  nips2015.tex


Suppose we have a dynamical system with latent variables $X_1,\ldots,X_T$ and observed variables $Y_1,\ldots,Y_T$ with observed values $y_1,\ldots,y_T$.  The system is described by the joint density:
\begin{align}
p(X_t|X_{1:t-1},Y_{1:t-1}) &= f(X_t|X_{1:t-1}) \\
p(Y_t|X_{1:t},Y_{1:t-1}) &= g(Y_t|X_{1:t})
\end{align}
where $X_0=x_0$ is some default initial value, and $f$ and $g$ are conditional densities.

Given observations $Y_{1:T}=y_{1:T}$, we will use a particle filter for posterior computation.  The $i$th particle will be denoted $x^i_1,\ldots, x^i_T$.  Particles are simulated and weighted at each stage $t=1,\ldots,T$:
\begin{align}
x^i_t|x^i_{t-1} &\sim q(\cdot|x^i_{t-1}) \\
w^i_t &= \frac{f(x^i_t|x^i_{t-1})g(y_t|x^i_t)}{q(x^i_t|x^i_{t-1})} \\
W^i_t &= W^i_{t-1} w^i_t 
\end{align}
where $q(\cdot|x)$ is the proposal density, $w^i_t$ is the weight associated with observation $y_t$, and $W^i_t$ is the weight of particle $i$ after stage $t$.  We can estimate probabilities of observations as follows:
\begin{align}
p(y_{1:t}) &\approx \frac{1}{N} \sum_{i=1}^N W^i_t \\
p(y_t|y_{1:t-1}) &\approx \frac{1}{N} \sum_{i=1}^N w^i_t
\end{align}

We will use a parallel computing architecture, where each particle is simulated on a separate thread.  In typical SMC algorithms with resampling, all particles have to be synchronized when a resampling step is considered.  Synchronizing many parallel threads is problematic and can lead to significant slowdown.  

We will consider a SMC algorithm which does not require synchronization.  The basic idea is that instead of resampling, we will consider particle branching, where each particle can result in 0 or more children.  These branching events happen asynchronously and mutually exclusively, i.e.\ they are processed one at a time.

At each stage $t$ of the particle filter, particles process observation $y_t$ in a mutually exclusive manner.  Without loss of generality, we can order the particles $1,2,\ldots$ in the order they process $y_t$.  This order need not be independent of the state of the particles $x^i_{1:t}$.

We keep track of the average weight associated with observation $y_t$ in an online manner:
\begin{align}
\overline{W}^i_t &= W^{i}_t &&\text{for $i=1$,}\\
\overline{W}^i_t &= \frac{i-1}{i} \overline{W}^{i-1}_t + \frac{1}{i} W^{i}_t 
&&\text{for $i=2,3,\ldots$.}
\end{align}
The number of children of particle $i$ should be dependent on the weight $W^{i}_t$ of particle $i$ relative to those of other particles.  The higher the weight, the more likely that this particle is located in a high posterior probability part of the space, so we should let this particle have more children, and vice versa.  

In an online asynchronous particle system as described here, we do not have access to the weights of future particles when processing $i$.  Instead we will compare $W^{i}_t$ to the current average weight $\overline{W}^i_t$ among particles processed thus far.  Specifically, the number of children, which we denote by $M^{i}_{t+1}$, will depend on
\begin{align}
R^i_t = \frac{W^{i}_t}{\overline{W}^i_t}
\end{align}
Each child of particle $i$ will get a weight $V^{i}_{t+1}$ such that the total weight of all children $M^{i}_{t+1}V^{i}_{t+1}$ has expectation $W^{i}_t$.  For example, if $M^i_{t+1}>0$ with certainty, we can use $V^{i}_{t+1}={W}^i_t/M^i_{t+1}$, while if the expectation of $M^i_{t+1}$ is $R^i_t$, we can use $V^i_{t+1}=\overline{W}^i_t$.  

Generally, we would like $M^i_{t+1}$ to be large when $R^i_t$ is large.  For example, $M^i_{t+1}$ can be independent of each other (conditioned on the weights), and be Poisson distributed with mean $R^i_t$.  Another possibility is to use the lowest variance integer-valued distribution with mean $R^i_t$, which takes values $\lfloor R^i_t\rfloor$ and $\lceil R^i_t\rceil$ with probabilities $\lceil R^i_t\rceil-R^i_t$ and $R^i_t-\lfloor R^i_t\rfloor$ respectively (if $R^i_t$ is integer-valued, $M^i_{t+1}=R^i_t$ deterministically).  

Suppose we start the system with $N_1=N$ particles.  The number of particles at subsequent stages $t$ is given recursively as:
\begin{align}
N_t &= \sum_{i=1}^{N_{t-1}} M^i_t &&\text{for $t=2,\ldots,T$.}
\end{align}
One issue with the above examples, where the number of children for each particle is conditionally independent, is that the variance of the total number of particles at each generation can grow without bound.  This can result in the number of particles becoming too large, or collapse to 1.

Instead, we will allow $M^i_t$ to depend on the number of children of previous particles, in such a way that we can stabilize the total number of particles at each generation.  Suppose that we wish for the number of particles to be stabilized around $N$.  After $i-1$ particles have been processed, we expect the total number of children produced at that point to be approximately $i-1$, so that if the number is less than $i-1$ we should allow particle $i$ to produce more children, and vice versa.  Similarly, if we already currently have more than $N$ children, we should allow particle $i$ to produce less children.  I have used the following scheme, which seems to work quite well:
\begin{align}
(M^i_{t+1},V^i_{t+1}) = \begin{cases}
(0,\overline{W}^i_t) \text{ w.p. $1-R^i_t$, }
	&\text{if $R^i_t<1$;} \\
(1,\overline{W}^i_t) \text{ w.p. $R^i_t$, } 
	&\text{if $R^i_t<1$;} \\
(\lfloor R^i_t\rfloor,\frac{W^i_t}{\lfloor R^i_t\rfloor})
	&\text{if $R^i_t\ge 1$ and $\sum_{j=1}^{i-1} M^j_{t+1}> \min(N,i-1)$;} \\
(\lceil R^i_t\rceil,\frac{W^i_t}{\lceil R^i_t\rceil})
	&\text{if $R^i_t\ge 1$ and $\sum_{j=1}^{i-1} M^j_{t+1}\le \min(N,i-1)$.}
\end{cases}
\label{eq:resampling_rule}
\end{align}




The observation probabilities can now be estimated as follows:
\begin{align}
p(y_t|y_{1:t-1}) &\approx \frac{1}{N_t} \sum_{i=1}^{N_t} w^i_t \\
p(y_{1:t}) = \prod_{s=1}^t p(y_s|y_{1:s-1})
&\approx \prod_{s=1}^t \frac{1}{N_s} \sum_{i=1}^{N_s} w^i_s
\end{align}
Note that since the number of particles at each stage is random, we have to estimate the overall observation probability using a product of estimates, one for each conditional probabilities.  

It should be possible to show that the estimators for the observation probabilities are unbiased.  In fact the claim should be that
\begin{align}
\sum_{i=1}^{N_t} W^i_t F(x^i_t)
\end{align}
is an unbiased estimator of 
\begin{align}
\int F(x) p(x|y_{1:t})dx
\end{align}
for well-behaving test function $F$.  Probably an argument by induction will work.

